Simplex QP-based methods for minimizing a conic quadratic objective over polyhedra

We consider minimizing a conic quadratic objective over a polyhedron. Such problems arise in parametric value-at-risk minimization, portfolio optimization, and robust optimization with ellipsoidal objective uncertainty; and they can be solved by polynomial interior point algorithms for conic quadratic optimization. However, interior point algorithms are not well-suited for branch-and-bound algorithms for the discrete counterparts of these problems due to the lack of effective warm starts necessary for the efficient solution of convex relaxations repeatedly at the nodes of the search tree. In order to overcome this shortcoming, we reformulate the problem using the perspective of the quadratic function. The perspective reformulation lends itself to simple coordinate descent and bisection algorithms utilizing the simplex method for quadratic programming, which makes the solution methods amenable to warm starts and suitable for branch-and-bound algorithms. We test the simplex-based quadratic programming algorithms to solve convex as well as discrete instances and compare them with the state-of-the-art approaches. The computational experiments indicate that the proposed algorithms scale much better than interior point algorithms and return higher precision solutions. In our experiments, for large convex instances, they provide up to 22x speed-up. For smaller discrete instances, the speed-up is about 13x over a barrier-based branch-and-bound algorithm and 6x over the LP-based branch-and-bound algorithm with extended formulations.

==> tables/continuousCard1000withnormalBisection.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Convex cardinality instances with $1,000$ variables.}
\begin{center}
\label{tab:contCard1000}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{} &\multirow{2}{*}{\texttt{Method}}&\multicolumn{3}{c|}{$\Omega=1$} &\multicolumn{3}{c|}{$\Omega=2$} &\multicolumn{3}{c}{$\Omega=3$} \\
$r$&$\alpha$&&\texttt{time}&\texttt{\#iter} &\texttt{\#QP}&\texttt{time}&\texttt{\#iter} &\texttt{\#QP}&\texttt{time}&\texttt{\#iter} &\texttt{\#QP} \\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.1}
&ALG1&1.0&22&20&1.1&53&24&1.3&104&29\\
&&ALG2&\textbf{0.8}&\textbf{41}&\textbf{14}&\textbf{0.9}&\textbf{95}&\textbf{15}&\textbf{0.9}&\textbf{150}&\textbf{15}\\
&&Bisection&1.1&38&26&1.2&95&29&1.3&120&31\\
&&BAR&4.6&16&-&4.9&24&-&5.2&26&-\\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.5}
&ALG1&1.1&33&23&1.1&69&24&1.5&144&37\\
&&ALG2&\textbf{0.8}&\textbf{60}&\textbf{14}&\textbf{0.9}&\textbf{125}&\textbf{15}&\textbf{0.9}&\textbf{200}&\textbf{15}\\
&&Bisection&1.2&48&30&1.3&117&33&1.4&192&33\\
&&BAR&4.5&21&-&5.1&25&-&5.8&29&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.1}&ALG1&0.9&33&19&1.1&73&25&1.2&110&25\\
&&ALG2&\textbf{0.8}&\textbf{49}&\textbf{14}&\textbf{0.9}&\textbf{126}&\textbf{14}&\textbf{0.9}&\textbf{172}&\textbf{14}\\
&&Bisection&1.2&57&30&1.3&115&31&1.4&176&31\\
&&BAR&4.7&22&-&4.5&22&-&5.1&25&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.5}&ALG1&1.0&48&22&1.1&99&22&1.2&151&25\\
&&ALG2&\textbf{0.9}&\textbf{94}&\textbf{14}&\textbf{0.9}&\textbf{179}&\textbf{14}&\textbf{1.0}&\textbf{233}&\textbf{15}\\
&&Bisection&1.3&78&31&1.4&149&33&1.5&244&33\\
&&BAR&4.4&21&-&4.9&24&-&5.2&26&-\\
\midrule
\multicolumn{2}{c|}{\multirow{3}{*}{avg}}&ALG1&1.0&34&21&1.1&73&24&1.3&127&29\\
&&ALG2&\textbf{0.8}&\textbf{61}&\textbf{14}&\textbf{0.9}&\textbf{131}&
\textbf{15}&\textbf{0.9}&\textbf{189}&\textbf{15} \\
&&Bisection&1.2&55&29&1.3&119&31&1.4&183&32\\
&&BAR&4.3&20&-&4.9&24&
-&5.3&27&- \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/continuousCard200.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for continuous cardinality instances with $200$ variables.}
\begin{center}
\label{tab:contCard200}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP} \\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.1}&ALG11&0.1&253&20&0.1&235&19&0.1&223&19\\
&&ALG12&0.1&15&19&0.1&31&21&0.1&52&21\\
&&ALG2&0.1&27&14&0.1&65&13&0.1&80&15\\
&&BAR&0.1&17&-&0.1&19&-&0.1&18&-\\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.5}&ALG11&0.1&299&17&0.1&286&19&0.1&277&22\\
&&ALG12&0.1&19&17&0.1&33&19&0.1&49&22\\
&&ALG2&0.1&26&14&0.1&53&14&0.1&77&14\\
&&BAR&0.1&20&-&0.1&20&-&0.1&18&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.1}&ALG11&0.1&340&17&0.1&331&15&0.1&322&16\\
&&ALG12&0.1&16&17&0.1&32&17&0.1&46&18\\
&&ALG2&0.1&30&13&0.1&48&13&0.1&71&13\\
&&BAR&0.1&20&-&0.1&23&-&0.1&18&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.5}&ALG11&0.1&368&15&0.1&356&16&&&\\
&&ALG12&0.1&20&16&0.1&37&17&&&\\
&&ALG2&0.1&35&13&0.1&55&13&&\\
&&BAR&0.1&21&-&0.1&24&-&&&-\\
\midrule
\multicolumn{2}{c|}{\multirow{4}{*}{\textbf{Average}}}&\textbf{ALG11}&\textbf{0.1}&\textbf{315}&\textbf{17}&\textbf{0.1}&\textbf{302}&
\textbf{17}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{ALG12}&\textbf{0.1}&\textbf{18}&\textbf{17}&\textbf{0.1}&\textbf{33}&\textbf{18}&\textbf{-}&\textbf{-}&\textbf{-}\\
&&\textbf{ALG2}&\textbf{0.1}&\textbf{30}&\textbf{13}&\textbf{0.1}&\textbf{55}&
\textbf{13}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{BAR}&\textbf{0.1}&\textbf{19}&\textbf{-}&\textbf{0.1}&\textbf{21}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/continuousGrid20.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for path instances with $760$ variables ($20\times 20$ grid).}
\begin{center}
\label{tab:contGrid20}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP} \\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.1}&ALG11&1.5&1,339&13&1.7&1,271&16&1.7&1,189&18\\
&&ALG12&0.8&347&14&1.0&468&16&1.3&570&20\\
&&ALG2&0.8&462&12&1.0&639&13&\textbf{1.1}&\textbf{732}&\textbf{13}\\
&&BAR&4.3&21&-&4.4&21&-&5.4&26&-\\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.5}&ALG11&1.6&1,492&12&1.7&1,421&14&1.9&1,317&19\\
&&ALG12&\textbf{0.7}&\textbf{321}&\textbf{12}&0.9&411&13&1.2&511&18\\
&&ALG2&0.8&419&11&0.9&584&12&\textbf{1.1}&\textbf{662}&\textbf{14}\\
&&BAR&4.5&22&-&4.5&22&-&3.4&16&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.1}&ALG11&1.6&1,423&12&1.7&1,340&15&1.8&1,278&14\\
&&ALG12&0.7&321&12&0.9&408&14&1.1&477&15\\
&&ALG2&0.7&379&11&0.9&545&11&1.1&680&13\\
&&BAR&5.3&26&-&4.3&22&-&4.6&24&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.5}&ALG11&1.8&1,398&16&1.8&1,368&14&1.9&1,327&15\\
&&ALG12&0.8&329&15&\textbf{0.9}&\textbf{391}&\textbf{14}&1.1&471&16\\
&&ALG2&\textbf{0.7}&\textbf{361}&\textbf{12}&1.0&537&12&1.1&641&13\\
&&BAR&3.7&24&-&3.6&22&-&2.9&17&-\\
\midrule
\multicolumn{2}{c|}{\multirow{4}{*}{\textbf{Average}}}&\textbf{ALG11}&\textbf{1.6}&\textbf{1,413}&\textbf{13}&\textbf{1.7}&\textbf{1,350}&
\textbf{14}&\textbf{1.9}&\textbf{1,278}&\textbf{17} \\
&&\textbf{ALG12}&\textbf{0.7}&\textbf{330}&\textbf{13}&\textbf{0.9}&\textbf{420}&\textbf{14}&\textbf{1.2}&\textbf{507}&\textbf{17}\\
&&\textbf{ALG2}&\textbf{0.7}&\textbf{405}&\textbf{12}&\textbf{0.9}&\textbf{576}&
\textbf{12}&\textbf{1.1}&\textbf{678}&\textbf{13} \\
&&\textbf{BAR}&\textbf{4.5}&\textbf{23}&\textbf{-}&\textbf{4.2}&\textbf{22}&
\textbf{-}&\textbf{4.1}&\textbf{21}&\textbf{-} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/continuousGrid40.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for path instances with $3,120$ arcs ($40\times 40$ grid).}
\begin{center}
\label{tab:contGrid40}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP}&\textbf{T}&\textbf{I} &\textbf{QP} \\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.1}&ALG11&55.0&7,115&15&57.5&6,683&21&&&\\
&&ALG12&17.2&1,305&14&25.5&1,846&21&&&\\
&&ALG2&\textbf{16.9}&\textbf{1,607}&\textbf{12}&\textbf{23.1}&\textbf{2,373}&\textbf{14}&&&\\
&&BAR&391.3&25&-&308.2&19&-&&&-\\
\midrule
\multirow{4}{*}{100}&\multirow{4}{*}{0.5}&ALG11&61.8&7,669&17&67.0&7,196&24&&&\\
&&ALG12&\textbf{16.1}&\textbf{1,288}&\textbf{14}&25.1&1,845&21&&&\\
&&ALG2&16.9&1,666&12&\textbf{23.5}&\textbf{2,403}&\textbf{13}&&&\\
&&BAR&344.9&21&-&297.1&17&-&&&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.1}&ALG11&72.4&7,408&14&74.2&7,108&19&&&\\
&&ALG12&\textbf{14.9}&\textbf{1,178}&\textbf{13}&\textbf{22.1}&\textbf{1,569}&\textbf{18}&&&\\
&&ALG2&16.1&1,423&12&22.7&2,273&13&&&\\
&&BAR&354.9&24&-&287.7&18&-&&&-\\
\midrule
\multirow{4}{*}{200}&\multirow{4}{*}{0.5}&ALG11&82.9&7,927&16&&&&&&\\
&&ALG12&\textbf{16.3}&\textbf{1,261}&\textbf{14}&&&&&&\\
&&ALG2&16.4&1,502&12&&&&&&\\
&&BAR&370.2&23&-&&&-&&&-\\
\midrule
\multicolumn{2}{c|}{\multirow{4}{*}{\textbf{Average}}}&\textbf{ALG11}&\textbf{68.0}&\textbf{7,530}&\textbf{16}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{ALG12}&\textbf{16.1}&\textbf{1,258}&\textbf{14}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{ALG2}&\textbf{16.6}&\textbf{1,550}&\textbf{12}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{BAR}&\textbf{365.3}&\textbf{23}&\textbf{-}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/discreteCard1000.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for discrete cardinality instances with $1,000$ variables.}
\begin{center}
\label{tab:discCard1000}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S} \\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.1}&BBA1&310&2,170&0.0\%/5&7,200&37,994&0.1\%/0&7,200&31,811&0.2\%/0\\
&&BBBR&5,254&810&0.0\%/2&7,200&1,082&0.1\%/0&7,200&1,340&0.6\%/0\\
&&CXSP&7,200&166&$\infty/0$&7,200&158&$\infty$/0&7,200&142&$\infty$/0\\
&&CXLP&6,787&104,125&0.0\%/1&7,200&151,288&0.2\%/0&7,200&213,903&0.6\%/0\\
&&CXLPE&413&4,843&0.0\%/5&7,200&47,429&0.1\%/0&7,200&30,673&0.3\%/0\\
&&CXD&\textbf{242}&\textbf{3,164}&\textbf{0.0\%/5}&\textbf{7,200}&\textbf{82,632}&\textbf{0.0\%/0}&7,200&50,018&0.2\%/0\\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.5}&BBA1&2,869&15,645&0.0\%/4&7,200&30,955&0.1\%/0&7,200&25,395&0.5\%/0\\
&&BBBR&7,200&1,186&0.1\%/0&7,200&800&0.3\%/0&7,200&1,304&1.3\%/0\\
&&CXSP&7,200&174&$\infty/0$&7,200&169&$\infty$/0&7,200&150&$\infty$/0\\
&&CXLP&7,200&117,108&0.1\%/0&7,200&162,201&0.3\%/0&7,200&318,337&1.8\%/0\\
&&CXLPE&2,596&26,156&0.0\%/4&7,200&40,191&0.2\%/0&7,200&32,858&0.6\%/0\\
&&CXD&\textbf{2,259}&\textbf{34,562}&\textbf{0.0\%/4}&7,200&56,787&0.1\%/0&\textbf{7,200}&\textbf{33,409}&\textbf{0.4\%/0}\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.1}&BBA1&\textbf{720}&\textbf{5,906}&\textbf{0.0\%/5}&7,200&43,332&0.1\%/0&7,200&35,227&0.2\%/0\\
&&BBBR&7,200&1,521&0.0\%/0&7,200&874&0.3\%/0&7,200&1,412&0.8\%/0\\
&&CXSP&7,200&160&$\infty/0$&7,200&148&$\infty$/0&7,200&151&$\infty$/0\\
&&CXLP&7,200&94,999&0.0\%/0&7,200&131,608&0.2\%/0&7,200&144,173&0.7\%/0\\
&&CXLPE&1,628&11,399&0.0\%/5&7,200&30,857&0.1\%/0&7,200&19,698&0.3\%/0\\
&&CXD&949&10,691&0.0\%/5&7,200&48,595&0.1\%/0&7,200&33,404&0.2\%/0\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.5}&BBA1&\textbf{1,106}&\textbf{8,594}&\textbf{0.0\%/5}&7,200&41,087&0.1\%/0&7,200&35,479&0.3\%/0\\
&&BBBR&6,215&1,175&0.2\%/1&7,200&1,310&0.5\%/0&7,200&1,238&1.0\%/0\\
&&CXSP&7,200&159&$\infty/0$&7,200&158&$\infty$/0&7,200&155&$\infty$/0\\
&&CXLP&7,200&100,590&0.0\%/0&7,200&126,281&0.3\%/0&7,200&169,065&0.7\%/0\\
&&CXLPE&1,772&12,456&0.0\%/4&7,200&30,293&0.1\%/0&7,200&20,626&0.4\%/0\\
&&CXD&1,498&16,897&0.0\%/5&7,200&48,951&0.1\%/0&7,200&29,059&0.3\%/0\\
\midrule
\multicolumn{2}{c|}{\multirow{6}{*}{\textbf{Average}}}&\textbf{BBA1}&\textbf{1,251}&\textbf{8,079}&\textbf{0.0\%/19}&\textbf{7,200}&\textbf{38,342}&
\textbf{0.1\%/0}&\textbf{7,200}&\textbf{31,978}&\textbf{0.3\%/0} \\
&&\textbf{BBBR}&\textbf{6,469}&\textbf{1,173}&\textbf{0.1\%/3}&\textbf{7,200}&\textbf{1,017}&
\textbf{0.3\%/0}&\textbf{7,200}&\textbf{1,324}&\textbf{0.9\%} \\
&&\textbf{CXSP}&\textbf{7,200}&\textbf{165}&\textbf{$\infty$/0}&\textbf{7,200}&\textbf{158}&
\textbf{$\infty$/0}&\textbf{7,200}&\textbf{149}&\textbf{$\infty$/0} \\
&&\textbf{CXLP}&\textbf{7,130}&\textbf{104,206}&\textbf{0.0\%/1}&\textbf{7,200}&\textbf{142,844}&
\textbf{0.3\%/0}&\textbf{7,200}&\textbf{211,370}&\textbf{0.9\%/0} \\
&&\textbf{CXLPE}&\textbf{1,602}&\textbf{13,714}&\textbf{0.0\%/18}&\textbf{7,200}&\textbf{37,192}&
\textbf{0.1\%/0}&\textbf{7,200}&\textbf{25,964}&\textbf{0.4\%/0} \\
&&\textbf{CXD}&\textbf{1,237}&\textbf{16,329}&\textbf{0.0\%/19}&\textbf{7,200}&\textbf{59,241}&
\textbf{0.1\%}&\textbf{7,200}&\textbf{36,472}&\textbf{0.3\%/0} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/discreteCard500.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\setlength{\tabcolsep}{2pt}
\begin{table}[h!]
\caption{Results for discrete cardinality instances with $500$ variables.}
\begin{center}
\label{tab:discCard500}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c c | c c c c| c c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Inst.}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{4}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{4}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{4}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{N} &\textbf{G}&\textbf{S}&\textbf{T}&\textbf{N} &\textbf{G}&\textbf{S}&\textbf{T}&\textbf{N} &\textbf{G}&\textbf{S} \\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.1}&BBA1&\textbf{16}&\textbf{510}&\textbf{0.0}&\textbf{5}&3,490&71,973
&0.0&3&7,200&117,830&0.3&0\\
&&BBBR&505&510&0.0&5&7,200&5,854&0.0&0&7,200&6,337&0.5&0\\
&&CXSP&922&634&0.0&5&7,200&4,500&0.1&0&7,200&4,348&0.6&0\\
&&CXLP&4,400&81,844&0.0&2&7,200&192,915&0.4&0&7,200&222,694&1.0&0\\
&&CXLPE&21&977&0.0&5&4,241&63,086&0.1&3&7,200&68,450&0.4&0\\
&&CXD&17&992&0.0&5&\textbf{2,750}&\textbf{73,256}&\textbf{0.0}&\textbf{4}&7,200&119,116&0.3&0\\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.5}&BBA1&175&4,256&0.0&5&\textbf{6,345}&\textbf{120,762}&\textbf{0.1}&\textbf{1}&7,200&114,948&0.4&0\\
&&BBBR&4,115&3,340&0.0&3&7,200&5,773&0.2&0&7,200&5,332&0.7&0\\
&&CXSP&5,085&3,224&0.0&2&7,200&4,338&0.3&0&7,200&4,221&1.0&0\\
&&CXLP&6,081&117,875&0.1&1&7,200&200,322&0.5&0&7,200&247,221&1.1&0\\
&&CXLPE&271&9,497&0.0&5&7,079&108,775&0.1&1&7,200&82,346&0.5&0\\
&&CXD&\textbf{173}&\textbf{8,361}&\textbf{0.0}&\textbf{5}&6,422&150,216&0.1&1&7,200&143,067&0.4&0\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.1}&BBA1&\textbf{18}&\textbf{593}&\textbf{0.0}&\textbf{5}&\textbf{5,020}&\textbf{122,236}&\textbf{0.0}&\textbf{3}
&\textbf{7,200}&\textbf{143,826}&\textbf{0.3}&\textbf{0}\\
&&BBBR&777&594&0.0&5&7,200&5,687&0.1&0&7,200&5,974&0.6&0\\
&&CXSP&1,411&828&0.0&5&7,200&4,196&0.2&0&7,200&4,306&0.6&0\\
&&CXLP&5,865&103,029&0.0&1&7,200&156,904&0.4&0&7,200&178,387&1.2&0\\
&&CXLPE&71&2,161&0.0&5&6,695&61,884&0.1&1&7,200&44,880&0.4&0\\
&&CXD&47&1,181&0.0&5&6,391&119,944&0.1&1&7,200&77,913&0.4&0\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.5}&BBA1&\textbf{208}&\textbf{7,476}&\textbf{0.0}&\textbf{5}&
\textbf{7,200}&\textbf{168,091}&\textbf{0.1}&\textbf{0}&-&-&-&-\\
&&BBBR&4,173&5,422&0.0&3&7,200&5,608&0.2&0&-&-&-&-\\
&&CXSP&4,299&2,751&0.1&3&7,200&4,355&0.3&0&-&-&-&-\\
&&CXLP&7,200&130,471&0.1&0&7,200&154,538&0.5&0&-&-&-&-\\
&&CXLPE&597&11,945&0.0&5&7,200&60,864&0.0&0&-&-&-&-\\
&&CXD&500&12,190&0.0&5&7,200&110,620&0.2&0&-&-&-&-\\
\midrule
\multicolumn{2}{c|}{\multirow{6}{*}{\textbf{Average}}}&\textbf{BBA1}&\textbf{104}&\textbf{3,209}&\textbf{0.0}&\textbf{20}&\textbf{5,514}
&\textbf{120,766}&\textbf{0.1}&\textbf{7}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{BBBR}&\textbf{2,392}&\textbf{2,467}&\textbf{0.0}&\textbf{16}&\textbf{7,200}&\textbf{5,731}&
\textbf{0.2}&\textbf{0}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXSP}&\textbf{2,929}&\textbf{1,859}&\textbf{0.1}&\textbf{15}&\textbf{7,200}&\textbf{4,347}&
\textbf{0.2}&\textbf{0}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXLP}&\textbf{5,887}&\textbf{108,305}&\textbf{0.1}&\textbf{4}&\textbf{7,200}&\textbf{176,170}&
\textbf{0.5}&\textbf{0}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXLPE}&\textbf{240}&\textbf{6,145}&\textbf{0.0}&\textbf{20}&\textbf{7,200}&\textbf{73,655}&
\textbf{0.1}&\textbf{5}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXD}&\textbf{184}&\textbf{5,681}&\textbf{0.0}&\textbf{20}&\textbf{5,692}&\textbf{113,509}&
\textbf{0.1}&\textbf{6}&\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/discreteGrid20.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for discrete path instances with $760$ variables.}
\begin{center}
\label{tab:discGrid20}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S} \\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.1}&BBA1&\textbf{31}&\textbf{119}&\textbf{0.0\%/5}&\textbf{217}&\textbf{765}&\textbf{0.0\%/5}&\textbf{718}&\textbf{2,386}&\textbf{0.0\%/5}\\
&&BBBR&380&118&0.0\%/5&2,028&657&0.0\%/5&6,566&2,134&0.7\%/2\\
&&CXSP&1,207&178&$0.0\%/5$&5,586&820&1.3\%/3&7,200&1,132&7.1\%/0\\
&&CXLP&49&1,287&0.0\%/5&1,171&23,636&0.0\%/5&7,200&66,642&6.1\%/0\\
&&CXLPE&46&231&0.0\%/5&466&1,501&0.0\%/5&2,004&4,845&0.0\%/5\\
&&CXD&152&109&0.0\%/5&298&585&0.0\%/5&918&2,943&0.0\%/5\\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.5}&BBA1&\textbf{25}&\textbf{88}&\textbf{0.0\%/5}&\textbf{151}&\textbf{521}&\textbf{0.0\%/5}&\textbf{548}&
\textbf{1,716}&\textbf{0.0\%/5}\\
&&BBBR&314&89&0.0\%/5&1,675&543&0.0\%/5&4,527&1,354&1.1\%/3\\
&&CXSP&945&114&$0.0\%/5$&4,446&693&0.6\%/4&7,200&1,176&6.6\%/0\\
&&CXLP&44&855&0.0\%/5&993&16,195&0.0\%/5&6,051&71,981&2.4\%/3\\
&&CXLPE&35&180&0.0\%/5&218&952&0.0\%/5&901&3,434&0.0\%/5\\
&&CXD&154&78&0.0\%/5&281&581&0.0\%/5&598&1,793&0.0\%/5\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.1}&BBA1&\textbf{29}&\textbf{110}&\textbf{0.0\%/5}&\textbf{237}&\textbf{949}&\textbf{0.0\%/5}&\textbf{1,060}
&\textbf{4,103}&\textbf{0.0\%/5}\\
&&BBBR&361&105&0.0\%/5&2,248&784&0.2\%/4&4,936&1,688&1.6\%/3\\
&&CXSP&1,246&174&$0.0\%/5$&4,592&675&1.4\%/3&7,166&1,092&10.3\%/1\\
&&CXLP&64&1,870&0.0\%/5&2,001&27,268&0.7\%/4&6,533&72,639&6.6\%/1\\
&&CXLPE&49&204&0.0\%/5&542&1,781&0.0\%/5&3,068&5,467&1.2\%/4\\
&&CXD&143&102&0.0\%/5&408&883&0.0\%/5&1,811&4,963&0.0\%/5\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.5}&BBA1&\textbf{13}&\textbf{42}&\textbf{0.0\%/5}&\textbf{95}&\textbf{336}&\textbf{0.0\%/5}&\textbf{527}
&\textbf{1,849}&\textbf{0.0\%/5}\\
&&BBBR&167&44&0.0\%/5&1,354&373&0.0\%/5&5,755&1,755&0.2\%/4\\
&&CXSP&713&99&0.0\%/5&5,306&740&0.0\%/5&7,200&1,137&14.8\%/0\\
&&CXLP&31&410&0.0\%/5&869&19,094&0.0\%/5&7,200&70,434&7.6\%/5\\
&&CXLPE&24&74&0.0\%/5&283&891&0.0\%/5&1,888&4,083&0.0\%/5\\
&&CXD&157&50&0.0\%/5&312&459&0.0\%/5&1,061&2,872&0.0\%/5\\
\midrule
\multicolumn{2}{c|}{\multirow{6}{*}{\textbf{Average}}}&\textbf{BBA1}&\textbf{24}&\textbf{90}&\textbf{0.0\%/20}&\textbf{175}&\textbf{643}&
\textbf{0.0\%/20}&\textbf{713}&\textbf{2,514}&\textbf{0.0\%/20} \\
&&\textbf{BBBR}&\textbf{306}&\textbf{89}&\textbf{0.0\%/20}&\textbf{1,826}&\textbf{590}&
\textbf{0.0\%/19}&\textbf{5,447}&\textbf{1,733}&\textbf{0.9\%/12} \\
&&\textbf{CXSP}&\textbf{1,028}&\textbf{141}&\textbf{0.0\%/20}&\textbf{4,982}&\textbf{732}&
\textbf{0.8\%/15}&\textbf{7,192}&\textbf{1,134}&\textbf{9.7\%/1} \\
&&\textbf{CXLP}&\textbf{47}&\textbf{1,105}&\textbf{0.0\%/20}&\textbf{1,259}&\textbf{21,548}&
\textbf{0.2\%/19}&\textbf{6,757}&\textbf{70,424}&\textbf{5.7\%/9} \\
&&\textbf{CXLPE}&\textbf{39}&\textbf{172}&\textbf{0.0\%/20}&\textbf{377}&\textbf{1,281}&
\textbf{0.0\%/20}&\textbf{1,965}&\textbf{4,457}&\textbf{0.3\%/19} \\
&&\textbf{CXD}&\textbf{151}&\textbf{85}&\textbf{0.0\%/20}&\textbf{325}&\textbf{627}&
\textbf{0.0\%/20}&\textbf{1,097}&\textbf{3,143}&\textbf{0.0\%/20} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/discreteGrid40.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for discrete path instances with $3,120$ variables.}
\begin{center}
\label{tab:discGrid40}
\SingleSpacedXI
\scalebox{0.9}{
\begin{tabular}{ c c | c | c c c | c c c | c c c} 
\hline \hline
\multicolumn{2}{c |}{\textbf{\textbf{Instance}}} &\multirow{2}{*}{\textbf{Method}}&\multicolumn{3}{c|}{$\boldsymbol{\Omega=1}$} &\multicolumn{3}{c|}{$\boldsymbol{\Omega=2}$} &\multicolumn{3}{c}{$\boldsymbol{\Omega=3}$} \\
$\boldsymbol{r}$&$\boldsymbol{\alpha}$&&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S}&\textbf{T}&\textbf{N} &\textbf{G/S} \\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.1}&BBA1&\textbf{894}&\textbf{125}&\textbf{0.0\%/5}&\textbf{6,302}&\textbf{713}&\textbf{1.9\%/1}&&&\\
&&BBBR&7,200&34&1.1\%/0&7,200&31&$\infty$/0&&&\\
&&CXSP&7,200&11&$\infty$\%/0&7,200&11&$\infty$/0&&&\\
&&CXLP&2,256&1,924&0.0\%/5&7,200&7,750&4.4\%/0&&&\\
&&CXLPE&1,676&295&0.0\%/5&7,200&1,112&3.9\%/0&&&\\
&&CXD&2,173&166&0.0\%/5&7,200&655&3.0\%/0&&&\\
\midrule
\multirow{6}{*}{100}&\multirow{6}{*}{0.5}&BBA1&\textbf{712}&\textbf{85}&\textbf{0.0\%/5}&7,200&800&1.7\%/0&&&\\
&&BBBR&6,690&29&0.8\%/1&7,200&31&$\infty$/0&&&\\
&&CXSP&7,200&10&$\infty$/0&7,200&13&$\infty$/0&&&\\
&&CXLP&2,883&3,371&0.0\%/4&7,200&7,287&5.6\%/0&&&\\
&&CXLPE&1,171&206&0.0\%/5&7,200&1,379&8.0\%/0&&&\\
&&CXD&1,900&94&0.0\%/5&\textbf{7,200}&\textbf{1,269}&\textbf{1.1\%/0}&&&\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.1}&BBA1&\textbf{937}&\textbf{133}&\textbf{0.0\%/5}&\textbf{6,346}&\textbf{891}&\textbf{2.5\%/2}&&&\\
&&BBBR&6,847&30&1.2\%/1&7,200&34&9.1\%/0&&&\\
&&CXSP&7,200&10&$\infty$/0&7,200&11&$\infty$/0&&&\\
&&CXLP&3,280&4,171&0.0\%/5&7,200&9,155&6.0\%/0&&&\\
&&CXLPE&2,925&444&0.0\%/5&7,054&1,003&18.9\%/1&&&\\
&&CXD&2,918&139&0.0\%/5&7,200&638&3.0\%/1&&&\\
\midrule
\multirow{6}{*}{200}&\multirow{6}{*}{0.5}&BBA1&\textbf{1,919}&\textbf{300}&\textbf{0.0\%/5}&&&&&&\\
&&BBBR&6,845&30&1.4\%/1&&&&&&\\
&&CXSP&7,200&9&$\infty$/0&&&&&&\\
&&CXLP&4,185&6,476&0.2\%/4&&&&&&\\
&&CXLPE&3,264&632&0.0\%/4&&&&&&\\
&&CXD&3,567&215&0.0\%/5&&&&&&\\
\midrule
\multicolumn{2}{c|}{\multirow{6}{*}{\textbf{Average}}}&\textbf{BBA1}&\textbf{1,115}&\textbf{161}&\textbf{0.0\%/20}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{BBBR}&\textbf{6,918}&\textbf{31}&\textbf{1.1\%/3}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXSP}&\textbf{7,200}&\textbf{10}&\textbf{$\infty$/0}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXLP}&\textbf{3,151}&\textbf{3,985}&\textbf{0.1\%/18}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXLPE}&\textbf{2,259}&\textbf{394}&\textbf{0.0\%/19}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
&&\textbf{CXD}&\textbf{2,639}&\textbf{154}&\textbf{0.0\%/20}&\textbf{-}&\textbf{-}&
\textbf{-}&\textbf{-}&\textbf{-}&\textbf{-} \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}
